Backstepping Stabilization of the Linearized Saint-Venant-Exner Model

Using the backstepping design, we achieve exponential stabilization of the coupled Saint-Venant-Exner (SVE) PDE model of water dynamics in a sediment-filled canal with arbitrary values of canal bottom slope, friction, porosity, and water-sediment interaction under subcritical or supercritical flow regime. The studied SVE model consists of two rightward convecting transport Partial Differential Equations (PDEs) and one leftward convecting transport PDE. A single boundary input control (with actuation located only at downstream) strategy is adopted. A full state feedback controller is firstly designed, which guarantees the exponential stability of the closed-loop control system. Then, an output feedback controller is designed based on the reconstruction of the distributed state with a backstepping observer. It also guarantees the exponential stability of the closed-loop control system. The flow regime depends on the dimensionless Froude number Fr, and both our controllers can deal with the subcritical (Fr < 1) and supercritical (Fr > 1) flow regime. They achieve the exponential stability results without any restrictive conditions in contrast to existing results.

==> redef.tex <==
\def\nd{\noindent}
\def\vs{\vspace}
\def\hs{\hspace}
\def\ic{\hookrightarrow}
\def\v{\breve}
\def\O{\Omega}
\def\o{\omega}
\def\s{\sigma}
\def\d{\delta}
\def\D{\Delta}
\def\l{\lambda}
\def\eps{\varepsilon}
\def\a{\alpha}
\def\b{\beta}
\def\G{\Gamma}
\def\g{\gamma}
\def\disp{\displaystyle}
\def\z{\zeta}
\def\e{\eta}
\def\k{\kappa}
\def\der{\partial}
\def\rg{\rangle}
\def\lg{\langle}
\def\izt{\int_0^t}
\def\VH{V_H(\omega)}
\def\izT{\int_0^T}
\def\io{\int_\omega}
\def\m{\mu}
\def\a{\alpha}
\def\S{\Sigma}
\def\Ka{\kappa}
\def\ka{\kappa}
\def\b{\beta}
\def\l{\lambda}
\def\g{\gamma}
\def\r{\rho}
\def\t{\tau}
\def\th{\theta}
\def\Th{\Theta}
\def\G{\Gamma}
\def\O{\Omega}
\def\o{\omega}
\def\d{\delta}
\def\z{\zeta}
\def\F{\phi}
\def\f{\varphi}
\def\e{\eta}
\def\te{\theta}
\def\na{\nabla}
\def\dpa{\partial}
\def\qs{\forall}
\def\rot{\mbox{rot}}
\def\D{\Delta}
\def\eps{\varepsilon}
\def\ep{\epsilon}
\def\hs{\hspace}
\def\vs{\vspace}
\def\div{\mbox{div}}
\def\td{\longrightarrow}
% Si on utilise les fontes de l'AMS
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newtheorem{theo}{Th\'eor\`eme}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{propo}{Proposition}[section]
\newtheorem{exple}{Exemple}[section]
\newtheorem{lem}{Lemme}[section]
\newtheorem{lemm}{Lemma}
\newtheorem{cor}{Corollaire}[section]
\newtheorem{rem}{Remarque}[section]
\newtheorem{remm}{Remark}
\newtheorem{com}{Commentaire}[section]
\newtheorem{defini}{Definition}[section]
\newtheorem{exo}{Exercice}[section]












































